Multispectral Compressive Imaging Strategies using Fabry-P\'erot Filtered Sensors

This paper introduces two acquisition device architectures for multispectral compressive imaging. Unlike most existing methods, the proposed computational imaging techniques do not include any dispersive element, as they use a dedicated sensor which integrates narrowband Fabry-P\'erot spectral filters at the pixel level. The first scheme leverages joint inpainting and super-resolution to fill in those voxels that are missing due to the device's limited pixel count. The second scheme, in link with compressed sensing, introduces spatial random convolutions, but is more complex and may be affected by diffraction. In both cases we solve the associated inverse problems by using the same signal prior. Specifically, we propose a redundant analysis signal prior in a convex formulation. Through numerical simulations, we explore different realistic setups. Our objective is also to highlight some practical guidelines and discuss their complexity trade-offs to integrate these schemes into actual computational imaging systems. Our conclusion is that the second technique performs best at high compression levels, in a properly sized and calibrated setup. Otherwise, the first, simpler technique should be favored.

==> algos.tex <==
% !TEX root =./hsics.tex
\subsection{Recovery Method}
\label{sec:algo}
In order to invert~\eqref{eq:forward_model} and find the estimate $\hat{\vx}$ of the MS cube, using the analysis-sparsity prior, we use the convex problem called $\ell_1$-analysis \cite{Candes2011c} with an additional range constraint $ \Rr \eqdef [x_{\mathrm{min}},x_{\mathrm{max}}]^n $, which reads
\begin{equation}
\label{eq:l1analysis}
\hat{\vx} \eqdef \argmin{ \tilde{\vx} \in \Rr } { \norm{ \mA \tilde{\vx} }_1 \quad \mbox{s.t.} \quad \norm{\vy - \mPhi  \tilde{\vx} }_2 \leq \epsilon}.
\end{equation}
The constrained form of the problem has the advantage, over its penalized Lagrangian form, of being easily interpretable in terms of noise level. A good noise estimate or, for synthetic experiments, a noise oracle is sufficient for setting the regularization parameter $\epsilon$. This greatly simplifies the parameter tuning step which can otherwise be cumbersome in such a high dimensional setup.

For solving \eqref{eq:l1analysis}, we use Algorithm 2 from \cite{Almeida2013}, which is an adaptation of ADMM \cite{Boyd2010} to problems of the form
\begin{equation}
\min_{ \vec{z} } \textstyle \sum_{j=1}^J g_j \pa{\mat{H}_j \vec{z}} ,
\end{equation}
where $g_j$ are convex lower-semicontinuous functions and $\mat{H}_j$ are linear operators. %such that
%$ \mat{G} \eqdef ({\mat{H}_1}^\tr, \dots, {\mat{H}_J}^\tr)^\tr $ has full column rank. 
For the algorithm to be of practical interest, it is preferable to have an efficient method to compute $\mat{H}_j \vec{z}$, ${\mat{H}_j}^* \vec{w}_j$  and $ \pa{\sum_{j=1}^J \mu_j {\mat{H}_j}^*\mat{H}_j}^{-1} \vec{z}$ for arbitrary $\vec{z}, \vec{w}_j$ and $\mu_j >0$. In addition, a fast computation of the \emph{proximal operators} associated to the functions $g_j$ is desirable.

In \cite{Almeida2013}, in order to make their deconvolution method more efficient, the authors propose to add the missing columns in the sensing operator to handle the borders and recover a block-circulant structure. Building over these ideas, as will be further explained for both architectures in Sections~\ref{sec:msvi-sensing} and~\ref{sec:msrc-sensing}, we can add rows and columns to $\mPhi$ to accelerate the computations. We define an \emph{extended} sensing matrix $\bar{\mPhi} \in \RR^{\bar{m} \times \bar{n}}$ (with $\bar{m}\geq m$ and $\bar{n} \geq n$) and corresponding \emph{restriction operators} $\Rm \in \{0,1\}^{m\times \bar{m}}$ and $\Rn \in \{0,1\}^{n\times \bar{n}}$ such that 
\begin{equation}
\label{eq:extended_Phi}
\mPhi  =\Rm \bar{\mPhi} \Rn^{\,*}.
\end{equation}
The additional rows and columns of the extended matrix are chosen to make sure that $\bar{\mPhi}^*\bar{\mPhi} + \mu \Id$ is easy to invert for any $\mu >0$.
Furthermore, the analysis transform $\mA$ described in the previous section is actually a scaled tight frame, \ie there exists a diagonal weighting matrix $\mat{\Om}$ such that $\mA \eqdef \mat{\Om}\tilde{\mA}$ and $\tilde{\mA}^*\tilde{\mA} = \Id$.
In order to make use of those interesting properties of $\mA$ and $\mPhi$, we first define
\begin{equation}
\bar{\mat{\Om}} \eqdef \begin{bmatrix} \mat{\Om} & \\  &  \mat{0}_{\bar{n} - n}\end{bmatrix} \quad \mbox{and} \quad 
\bar{\mA} \eqdef \begin{bmatrix} \tilde{\mA}\Rn \\  \Rnc  \end{bmatrix},
\end{equation}
where $\Rnc \in \{0,1\}^{ (\bar{n} - n) \times \bar{n} } $ is the complementary restriction of $\Rn$ and $ \mat{0}_{\bar{n} - n}$ is the matrix of zeros of size $\bar{n} - n$ by $\bar{n} - n$. This ensures that the tight frame property $\bar{\mA}^*\bar{\mA} = \Id$ is preserved.
Let $ \bar{\vx} \eqdef \Rn^{\,*} \tilde{\vx}$, \ie a zero-padded version of $\tilde{\vx}$, and let $\bar{\val} \eqdef \bar{\mA} \bar{\vx}$ and $\bar{\vw} \eqdef \bar{\mPhi} \bar{\vx}$. Note that $\norm{\bar{\mat{\Om}}\bar{A} \bar{\vx} }_1 = \norm{A \tilde{\vx} }_1$ and $\norm{\vy - \Rm \bar{\mPhi} \bar{\vx} }_2 = \norm{\vy - \mPhi \tilde{\vx} }_2$.
The problem \eqref{eq:l1analysis} is then equivalently split in $J=3$ functions, namely, 
\begin{align}
g_1(\bar{\val}) &\eqdef \norm{ \bar{\mat{\Om}} \bar{\val}}_1  &\mbox{with }  &\mat{H}_1 \eqdef \bar{\mA} \\
g_2(\bar{\vw}) &\eqdef \iota_{\norm{\vy - \cdot} \leq \epsilon} (\Rm \bar{\vw})  &\mbox{with }  &\mat{H}_2 \eqdef \bar{\mPhi}\\
g_3(\bar{\vx}) &\eqdef \iota_{\Rr}(\Rn \bar{\vx})+\iota_{\{\vec{0}\}} (\Rnc \bar{\vx})  &\mbox{with }  &\mat{H}_3 \eqdef \Id,
\end{align} 
where $\iota_{\norm{\vy - \cdot}\leq \epsilon}$ denotes the indicator function of the constraint set $\enscond{\vw}{\norm{\vy - \vw} \leq \epsilon}$, $\iota_{\Rr}$ denotes the indicator of the range constraint and $\iota_{\{\vec{0}\}}$, the indicator of the $\{\vec{0}\}$ set. The corresponding proximal operators all admit a very simple closed form expression that can be efficiently evaluated. See, for instance \cite{Combettes2009} for more details on this.
Moreover, we have
\begin{equation}
\label{eq:sum_of_operators}
\textstyle\sum_{j=1}^3 \mu_j {\mat{H}_j}^*\mat{H}_j = \mu_1\pa{ \bar{\mPhi}^*\bar{\mPhi} + \tfrac{\mu_2 + \mu_3}{\mu_1} \Id},
\end{equation}
which, as required, is easily invertible.
Note that the resulting optimization is carried out with respect to the extended variable $\bar{\vx} \in \RR^{\bar{n}}$ but because $g_3(\bar{\vx}) $ imposes $\Rnc \bar{\vx} = \vec{0}$, it is equivalent to solving~\eqref{eq:l1analysis} with $\tilde{\vx} =  \Rn \bar{\vx}$.


%\begin{algorithm}[t]
%\caption{Alternating Direction Method of Multipliers}\label{alg:admm}
%\begin{algorithmic}[1]
%\Procedure{ADMM}{}\\
%\algorithmicrequire{ $\vx^{\iter{0}}$ }
%\State plop;
%\While{not done}
%\State plip;
%\EndWhile
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
